FastJAM: a Fast Joint Alignment Model for Images

Joint Alignment (JA) of images aims to align a collection of images into a unified coordinate frame, such that semantically-similar features appear at corresponding spatial locations. Most existing approaches often require long training times, large-capacity models, and extensive hyperparameter tuning. We introduce FastJAM, a rapid, graph-based method that drastically reduces the computational complexity of joint alignment tasks. FastJAM leverages pairwise matches computed by an off-the-shelf image matcher, together with a rapid nonparametric clustering, to construct a graph representing intra- and inter-image keypoint relations. A graph neural network propagates and aggregates these correspondences, efficiently predicting per-image homography parameters via image-level pooling. Utilizing an inverse-compositional loss, that eliminates the need for a regularization term over the predicted transformations (and thus also obviates the hyperparameter tuning associated with such terms), FastJAM performs image JA quickly and effectively. Experimental results on several benchmarks demonstrate that FastJAM achieves results better than existing modern JA methods in terms of alignment quality, while reducing computation time from hours or minutes to mere seconds. Our code is available at our project webpage, https://bgu-cs-vil.github.io/FastJAM/

==> figures/intro_fig.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    node distance=0.8cm and 0.8cm, 
    box/.style={draw=black, rounded corners, fill=blue!10, minimum width=2.5cm, minimum height=3.5cm},
    imgbox/.style={draw=none, fill=orange!10, rounded corners},
    point/.style={circle, draw=black, inner sep=1.2pt},
    arrow/.style={thick, -{Latex[round]}},
    every node/.style={font=\scriptsize},
    every path/.style={draw=black!60}
]

\foreach \x/\y/\name/\col in {
    0/2/A1/red,
    -0.6/2.6/A2/blue,
    -0.6/1.4/A3/green,
    0.6/2.6/A4/orange,
    0.6/1.4/A5/teal
}{
    \node[point, fill=\col] (\name) at (\x,\y) {};
}
\draw[imgbox] (-1.2,1.1) rectangle (1.2,3.0);
\node at (0,3.2) {Input Graph};

\foreach \x/\y/\name/\col in {
    2.2/2/B1/red,
    1.6/2.6/B2/blue,
    1.6/1.4/B3/green,
    2.8/2.6/B4/orange,
    2.8/1.4/B5/teal
}{
    \node[point, fill=\col] (\name) at (\x,\y) {};
}
\draw[imgbox] (1.4,1.1) rectangle (3.4,3.0);

\foreach \a/\b in {A1/B1, A2/B2, A3/B3, A4/B4, A5/B5} {
    \draw[dashed] (\a) -- (\b);
}

\draw[arrow] (3.5,2) -- (4.2,2);

%%% --- GRAPHSAGE BLOCK ---
\node[box, anchor=west] at (4.2,0.5) (graphsage) {};
\node at (5.45,3.3) {\textbf{GraphSAGE}};
\node at (5.45,3.0) {Full Graph};

\foreach \x/\y/\name/\col in {
    4.6/2.7/C1/red,
    5.5/2.6/C2/blue,
    5.1/2.0/C3/orange,
    4.8/1.4/C4/green,
    5.9/1.6/C5/yellow,
    5.7/0.9/C6/brown
}{
    \node[point, fill=\col] (\name) at (\x,\y) {};
}
\foreach \a/\b in {C1/C2, C1/C3, C2/C3, C3/C4, C3/C5, C5/C6, C4/C6} {
    \draw[dashed] (\a) -- (\b);
}

\draw[arrow] (6.8,2) -- (7.5,2);

\node[box, anchor=west, minimum width=2.2cm, minimum height=2.5cm] at (7.5,1.0) (pool) {};
\node at (8.6,3.3) {Pooling \&};
\node at (8.6,3.0) {Regression};

\foreach \x/\y/\name/\col in {
    8.0/2.2/P1/orange,
    9.2/2.2/P2/blue,
    8.0/1.2/P3/yellow,
    9.2/1.2/P4/brown
}{
    \node[point, fill=\col] (\name) at (\x,\y) {};
}
\foreach \a/\b in {P1/P2, P1/P3, P2/P4, P3/P4} {
    \draw (\a) -- (\b);
}

\draw[arrow] (9.6,2) -- (10.2,2);

\foreach \y/\col in {2.3/orange, 2.0/yellow, 1.7/brown} {
    \node[point, fill=\col, minimum size=6pt] at (10.4,\y) {};
}
\node[align=center] at (10.8,2.0) {Homography\\Prediction};

\end{tikzpicture}
\caption{FastJAM architecture. GraphSAGE propagates information from sparse keypoints to produce per-image homography predictions.}
\label{fig:fastjam}
\end{figure}


==> figures/method_fig.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[scale=0.4]{figures/images/fastjam_method_inital_figure.png}
    \caption{Initial Method Figure, Pipeline.}
    \label{Fig:Method}
\end{figure*}

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}
\newcommand{\WHITE}[1]{{{\color{white}{#1}}}}  

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{ForestGreen}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  
\newcommand{\PURPLE}[1]{{{\color{purple}{#1}}}}  
\newcommand{\SEAGREEN}[1]{{{\color{SeaGreen}{#1}}}}  
\newcommand{\NAVYBLUE}[1]{{{\color{NavyBlue}{#1}}}} 
\newcommand{\ORCHID}[1]{{{\color{Orchid}{#1}}}} 


\newcommand{\gr}[1]{{{\color{gray}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}

% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}
\newcommand{\ERAN}[1]{\RED{[ERAN: #1]}}

\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}


\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}}


% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

